Search for the critical point of strongly interacting matter

The existence and location of the QCD critical point is an object of both experimental and theoretical studies. The comprehensive data collected by NA61/SHINE during a two-dimensional scan in beam momentum (13A-150A GeV/c) and system size (p+p, p+Pb, Be+Be, Ar+Sc, Xe+La, Pb+Pb) allows for a systematic search for the critical point-a search for a non-monotonic dependence of various correlation and fluctuation observables on collision energy and size of colliding nuclei. In particular, fluctuations of particle number in transverse momentum space are studied. They are quantified by measuring the scaled factorial moments of multiplicity distribution.

==> sections/Analysis.tex <==
\section{Analysis}
\label{sec:analysis}

The goal of the analysis was to search for the critical point of the strongly interacting matter
by measuring the second scaled factorial moment for a selection of protons produced in central
\ArSc interactions at 150\AGeVc, using statistically independent points and cumulative variables.


\subsection{Statistically-independent data points}

The intermittency analysis yields the dependence of scaled factorial moments on
the number of subdivisions of transverse-momentum and cumulative transverse-momentum intervals.
In the past, the same data set was used for the analysis performed for different subdivision numbers.
This resulted in statistically-correlated data points; thus, the full covariance matrix is required
for proper statistical treatment of the results. The latter may be numerically not trivial~\cite{Wosiek:1990kw}.
For the first time,
statistically-independent data subsets were used to obtain results for each subdivision number.
In this case, the results for different subdivision numbers are statistically independent.
Only diagonal elements of the covariance matrix are non-zero, and thus the full relevant information
needed to interpret the results is
easy to present graphically and use in the statistical tests.
However, the procedure decreases the number of events used to calculate each data point increasing
statistical uncertainties.

The event number in a subset was selected to obtain similar values of the statistical uncertainties of results for different subsets.
Table~\ref{tab:fraction-of-events} presents a fraction of all available events used to calculate each of the 10 points.
\begin{table}[!ht]
    \centering
    \caption{
        Fraction of the total number of analyzed events used to calculate the second scaled
        factorial moments for the chosen number of cumulative momentum bins.
    }
    \vspace{1ex}
    \begin{tabular}{ l | c | c | c | c | c | c | c | c | c | c }
        number of bins          & 1   & 50 & 70 & 86 & 100 & 111 & 122 & 132 & 141 & 150 \\ \hline
        fraction of all events (\%) & 0.5 &  3.0 &  5.0 &  7.0 &   9.0 &  11.0 &  13.0 & 15.5 & 17.0 &  19.0
    \end{tabular}
    \label{tab:fraction-of-events}
\end{table}

\subsection{Uncertainties and biases}

The standard expression for the scaled factorial moments,
Eq.~\ref{eq:scaled-factorial-moments} can be rewritten as
\begin{equation}
\label{eq:sfm}
    F_{2}(M) = 2M^{2}\frac{\AVG{N_{2}(M)}}{\AVG{N}^{2}},
\end{equation}
where $N_{2}(M)$ denotes a total number of particle pairs in $M$ bins in an event.
Then the statistical uncertainties can be calculated using the standard error propagation:
\begin{equation}
    \frac{\sigma_{F_{2}}}{|F_{2}|} = \sqrt{\frac{(\sigma_{N_{2}})^{2}}{\AVG{N_{2}^{2}}}
    + 4\frac{(\sigma_{N})^{2}}{\AVG{N}^{2}}
    - 4\frac{(\sigma_{N_{2}N})^{2}}{\AVG{N}\AVG{N_{2}}}}.
\end{equation}





